A Theoretical View on Sparsely Activated Networks

Deep and wide neural networks successfully fit very complex functions today, but dense models are starting to be prohibitively expensive for inference. To mitigate this, one promising direction is networks that activate a sparse subgraph of the network. The subgraph is chosen by a data-dependent routing function, enforcing a fixed mapping of inputs to subnetworks (e.g., the Mixture of Experts (MoE) paradigm in Switch Transformers). However, prior work is largely empirical, and while existing routing functions work well in practice, they do not lead to theoretical guarantees on approximation ability. We aim to provide a theoretical explanation for the power of sparse networks. As our first contribution, we present a formal model of data-dependent sparse networks that captures salient aspects of popular architectures. We then introduce a routing function based on locality sensitive hashing (LSH) that enables us to reason about how well sparse networks approximate target functions. After representing LSH-based sparse networks with our model, we prove that sparse networks can match the approximation power of dense networks on Lipschitz functions. Applying LSH on the input vectors means that the experts interpolate the target function in different subregions of the input space. To support our theory, we define various datasets based on Lipschitz target functions, and we show that sparse networks give a favorable trade-off between number of active units and approximation quality.

==> Hybrid Sparsity (arxiv)/abstract.tex <==
\begin{abstract}
    Deep and wide neural networks successfully fit very complex functions today, but dense models are starting to be prohibitively expensive for inference. To mitigate this, one promising direction is networks that activate a sparse subgraph of the network. The subgraph is chosen by a data-dependent routing function, enforcing a fixed mapping of inputs to subnetworks (e.g., the Mixture of Experts (MoE) paradigm in Switch Transformers). 
    %However, there is no theoretical grounding for these sparsely activated models. 
    \rebut{However, prior work is largely empirical, and while existing routing functions work well in practice, they do not lead to theoretical guarantees on approximation ability.}
    \rebut{We aim to provide a theoretical explanation for the power of sparse networks.}
    As our first contribution, we present a formal model of data-dependent sparse networks that captures salient aspects of popular architectures.
    \rebut{We then introduce a routing function based on locality sensitive hashing (LSH) that enables us to reason about how well sparse networks approximate target functions.}
    \rebut{After representing LSH-based sparse networks with our model, we prove that sparse networks can match the approximation power of dense networks on Lipschitz functions.} 
    \rebut{Applying LSH on the input vectors means that the experts interpolate the target function in different subregions of the input space.}
    % The sparse networks use much fewer inference operations than dense networks, leading to a faster forward pass.
    % \rebut{Our constructions and analyses provide a theoretical explanation for why sparse networks work well in practice.}
    %Then, we show how to construct sparse networks that provably match the approximation power and total size of dense networks on Lipschitz functions. The sparse networks use much fewer inference operations than dense networks, leading to a faster forward pass. 
    % The key idea is to use locality sensitive hashing on the input vectors and then interpolate the function in subregions of the input space. This offers a theoretical insight into why sparse networks work well in practice. 
    \rebut{To support our theory, we define various datasets based on Lipschitz target functions, and we show that sparse networks give a favorable trade-off between number of active units and approximation quality.}
    %Finally, we present empirical findings that support our theory; compared to dense networks, sparse networks give a favorable trade-off between number of active units and approximation quality.
\end{abstract}

==> Hybrid Sparsity (arxiv)/conclusion.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Conclusion}
\label{sec:conclusion}

We provided the first systematic theoretical treatment of modern sparsely activated networks. To do so, we introduced the $\DSM$ model, which captures the sparsity in Mixture of Experts models, such as Switch and Scaling Transformers. We showed that $\DSM$ can simulate popular architectures as well as LSH-based networks. Then, we exhibited new constructions of sparse networks.
% , and proved that they approximate Lipschitz functions supported on general manifolds. 
% Our results match the power and size of dense networks, while requiring much fewer inference operations. 
Our use of LSH to build these networks offers a theoretical grounding for sparse networks.
% work well in practice. 
We complemented our theory with experiments, showing that sparse networks can approximate various functions.

For future work, it would be interesting to implement LSH-based networks in transformers for language/vision tasks. A related question is to determine the best way to interpolate in each LSH bucket (e.g., a higher degree polynomial may work better). 
% Another direction is to  understand how training of the lower layer can improve the representation power of sparse models. A final question is to theoretically analyze the training dynamics of the DSM model with SGD (similar to the results in~\cite{daniely2020learning} for learning parities).
Another question is whether a dense model is more powerful than a sparse model with the same number of total trainable parameters. Theorem~\ref{thm:main-lipschitz-lsh-ub} only says that a sparse model with similar number of parameters as a dense model can more efficiently (fewer FLOPs) represent Lipschitz functions. This does not say \emph{all} functions expressible by a dense model are also expressible by a sparse model. This is non-trivial question as $A^x$ depends on the input (i.e., $\DSM(d,t,t)$ may be more expressive than the dense model with width $t$).
We expect that dense networks can be trained to perform at least as well as sparse networks, \emph{assuming the width is large enough}. The dense networks should optimize the weights in the last layer to approximate the function, but they may not favor certain neurons depending on the input.

% \begin{enumerate}
%     \item talk about other directions for sparsely activated subgraphs. some mention of this in related work too?
%     \item 
% \end{enumerate}

% \subsection{Open Questions}

% Ideas for generalization to larger function class.
% Chebyshev polynomials. Tradeoff $\epsilon$ error do we need $(1/\epsilon)^k$ size because we need to store all of the coefficients. Can we prove a lower bound? If you store the first few coefs. Store $exp(k)$ coefs, not dependence on $\epsilon$. Can compute the contribution later coefs, and they should be negligible. This should be analyzed already in numerical analysis, especially for 1D and interpolation with small storage.

% Lower bound should also be tight for brownian motion or GRF but not tight for analytic functions. For polynomials can you do $\mathrm{poly}(k,1/\epsilon)$ size for $\epsilon$ error?

% What is the optimal way to interpolate within the bucket? We can have a constant function, we can have linear $ax + b$, or we can have a higher order polynomial.

% Can we prove a lower bound that is a function of the degree of the polynomial instead of the dimensionality? Because we need to capture the ups and downs for interpolation. Random values on the grid points, and see how many buckets we need.

% \subsection{TODO items for this paper}

% Can we write out the optimization problem and show that it is linear and hence convex.

% Check that we can prove that the derivatives are bounded for the real valued extension of the boolean Fourier expansion. What are the derivatives of the this function on $[-1,1]^d$ instead of just $\{-1,1\}^d$.

% What is the difference between spherical LSH and hyperplane LSH in our set-up and results?

% What is the optimal way to interpolate within the bucket? We can have a constant function, we can have linear $ax + b$, or we can have a higher order polynomial. What do we choose and why?

==> Hybrid Sparsity (arxiv)/dsm_vs_dense.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Data-Dependent Sparse Models are Less Expressive than Dense Models}
\label{sec:lshpower}
First we establish formally that the dense model is strictly more powerful than the sparse model when given the same width. Simple intuition tells this and this is formalized in the form of Lemmas \ref{lem:dense-expresses-lsh} and \ref{lem:lsh-doesnot-express-dense}.
% To start off with, some observations comparing the representation power of LSH tables vs 1-hidden layer ReLU networks (TLDR: When comparing LSH with table size $M$ and dense ReLU network with hidden width $M$, dense ReLU networks are strictly more expressive than LSH tables)
\begin{lemma}
\label{lem:dense-expresses-lsh}
Given a function $f$ which is expressible using a hyperplane-LSH with table size $M$, there exists a two layer ReLU network of hidden width $M$ which computes $f$. For an LSH parameter $\epsilon$, the norm of the weights in the top layer of the ReLU network will grow as $g(1/\epsilon)$.
\end{lemma}
\begin{proof}
Every entry in the table of the LSH model corresponds to a region in $\mathbb{R}^d$ which corresponds to $\log M$ hyper-plane inequalities being satisfied. 
\end{proof}

\begin{lemma}
\label{lem:lsh-doesnot-express-dense}
The other way around does not hold. Can we use a counting argument (info theoretic LB)? Naive argument on total number of parameters used to represent the function won't work as sparse model has equal (or more) total number of parameters.
Easier goal to prove: there exists a function which can be computed exactly in dense model but can't be exactly computed in sparse model.
Nicer goal: exists a function which can be computed exactly in dense model but can't even be approximated well in sparse model.
%The ability to train the bottom layer of the ReLU network will imply a separation between functions computable using LSH vs those computable using ReLU networks. (see Learning Parities with Neural Networks paper)
\end{lemma}
\begin{proof}

\end{proof}

If allowed sparsity level is much smaller than the input dimension $d$, then the sparse layer might have significantly more limited expressive power as compared to the more dense layer.
Consider a simple linear function which depends on only one of the $d$ input coordinates. (e.g. $f(x) = x_0$.)
\begin{enumerate}
\item Case 1: With a random ReLU layer of width $d/\epsilon^2$ followed by a dense layer on top, we get that we can learn this function. In case we remove the ReLU completely this is easier to see. we compute as our final layer weights $\{ 1/w_{0j}\}_{j=1}^{d/\epsilon^2}$. This will ensure that the $x_0$ component is present in all neurons and in the averaging process the coefficients of other coordinates vanish to 0.
What happens with the ReLU present? for each $x$, approximately half of the neurons will be active and the convergence still goes through at the same asymptotic rate. \nishanth{with ReLU present it is not clear that the other coordinates effect will vanish to 0. since they will only show up at second layer if activation is positive. need to think more carefully}
\item Case 2: With random ReLU layer of width $W$ followed by a $k$-sparse final layer, this is much harder. how large does $W$ need to be? \nishanth{unfinished argument}
$k=d$ trivially solves the problem as it reduces to above case.
\item Case 3: With trainable ReLU layer of width W followed by a $k$-sparse final layer, ... TBF
\end{enumerate}





==> Hybrid Sparsity (arxiv)/experiments.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Experiments}
\label{sec:experiments}

% Firstly we aim to show that using a random hash function based routing algorithm (used in this FB paper~\cite{roller2021hash}) for experts is sub-optimal for learning polynomials compared to an LSH based routing algorithm:
% \begin{enumerate}
%     \item Architecture A: 1st layer random ReLU of width $m$, dense linear layer 
%     \item Architecture B: first layer is random ReLU of width $m$, $k$-sparse linear layer per example. (the function to determine which $k$ to turn on is given by an LSH function with table size $m$ which maps the example $x$ to $k$ buckets).
%     \item Architecture C: 1st layer random ReLU of width $m$, $k$-sparse linear layer per example (the function to determine which $k$ to turn on is given by random hash function (not locality-sensitive) (closer to what is being done in the Hash Layers for Large Sparse Models paper.
%     \item Architecture D: 1st layer random ReLU of width $m$, $k$-sparse linear layer per example (the function to determine which $k$ to turn on is given by a hash function that is tailored to the dataset, e.g., we cluster the input space and then we hash all inputs in the same clusters to the same place)
% \end{enumerate}
% Evaluation metrics:
% \begin{enumerate}
%     \item Estimate the $\ell_\infty$ distance between the learned function and the ground truth function (max distance btw $f$ and approximation $\tilde f$)
%     \item Estimate the $\ell_2$ distance between the learned function and the ground truth function (MSE)
%     \item Scalability in dimension $d = 1, 2, \ldots, d_\mathrm{max}$
%     \item Scalability in sparsity $k = 1, 2, \ldots, k_\mathrm{max}$ (does it make sense to have $k_\mathrm{max} > d$?)
% \end{enumerate}
% Datasets (start with $d = 1$ for now):
% \begin{enumerate}
%     \item Synthetic: Brownian motion $f:[0,1]^d \to \mathbb{R}$
%     \item Synthetic: Some sort of smoothed Brownian motion $f:[0,1]^d \to \mathbb{R}$
%     \item Synthetic: Random degree $t$ polynomial where the inputs come from a random $k$ dimensional subspace
%     \item Synthetic: Random degree $t$ polynomial where the inputs only depend on $k$ random features (special case where $d-k$ coordinates are zero). 
%     \item Synthetic: Random degree $k$ polynomial where the inputs only depend on $k$ features. Specifically, $\pm 1$ coefs and inputs $\{-1,1\}^k$ and scale by $2^{k/2}$ so function is bounded in $\ell_2$. (special case where $t = k$ from above and inputs/coefs restricted to $\pm 1$)
%     \item Synthetic: Radially symmetric polynomial. Random polynomial $f:[0,1] \to \mathbb{R}$ where you evaluate $g(x) = f(x_{i_1} + \ldots + x_{i_k})$ where $i_1,\ldots,i_k \in [d]$ are randomly chosen.
%     \item Real: what are relevant real datasets here?
% \end{enumerate}    
   
% \subsection{Random Taylor Series}
% Fix degree, random coefs $\pm 1 / i!$. Differential everywhere, so smaller class than truly random function.

% If input value is in $[0,m]$, then coefs after $i \gg em$ are not important because negligible contribution after this point, for example, $(m)^{10\cdot em}/(em)! \ll 1$, where the value 10 can be optimized to be made smaller depending on the $\epsilon$ desired for approximation.

%\nishanth{Pose the experimental result on random hash performance reaching the same as sparse and dense models at high number of units activated as a conjecture for why Hash Layers paper works?}

To empirically verify our theoretical findings, we align our experiments with our proposed models and compare dense models, data-dependent sparse models ($\DSM$), LSH models, and sparse models with random hash based sparse layers. While $\DSM$ and LSH models are analyzed in the previous section, random hash based layers introduce sparsity with a random hash function, as an alternative of learnable routing modules and LSH in MoE models \cite{roller2021hash}. 
Our goal is to show that the $\DSM$ and $\LSH$ models achieve small MSE while using much fewer activated units than dense models. We also report similar observations on the CIFAR-10 dataset.

\subsection{Experimental set-up} 

\mypar{Models.} We compare dense models and three sparse models that cover a wide range of possible routing methods (Top-$K$ $\DSM$, $\LSH$, and random). We use Top-$K$ routing as a representative $\DSM$ model; it uses the $K$ largest activations, which depends on the input (see Section~\ref{sec:model-results}).
Dense, $\DSM$ and random hash sparse models contain a random-initialized, non-trainable bottom layer. 
For the random hash model, we uniformly choose a subset of the units.
%We use a random hash layer for random hash models to enforce sparsity. 
All networks have a trainable top layer. $\LSH$ models have non-trainable hyperplane coefficients for hashing and a trainable scalar in each bucket (this is the network output for inputs in that bucket). For ablations, we vary the number of hidden units and sparsity levels.

%The main difference between the $\DSM$ and $\LSH$ models is that $\DSM$ model is {\color{red} TODO Can you finish this sentence?} The model arch should be clear from the above description.

\mypar{Data.} 
Our main goal is to empirically evaluate the construction from Theorem~\ref{thm:main-lipschitz-lsh-ub}, while comparing routing functions. To align with our theory, we consider Lipschitz target functions. We synthetically construct the data with two functions that are common bases for continuous functions: random low-degree polynomials and random hypercube functions. Both are normalized to be $L$-Lipscthiz for $L = O(1)$. We also present results on a real dataset, CIFAR-10, which corroborates our findings from the synthetic data experiments.
% We evaluate with synthetic data from two random, Lipschitz target functions that are commonly used basis functions for arbitrary continuous functions. 

\mypar{Random polynomial.} $p(x)$ of degree $D$ for $x \in \mathbb{R}^d$ with sum of coefficient absolute values \rebut{$< 1/D$}. \rebut{ As a result, we ensure that the function is 1-Lipschitz over $[-1,1]^d$.}

\mypar{Random hypercube function.} $f: [-1, 1]^d \rightarrow \mathbb{R}$ which interpolates the indicator functions at each corner with random $\{-1, 1\}$ value at each corner. Concretely, the function is defined as follows: for each corner point $y \in \{-1, 1\}^d$, its indicator function is $I_y(x) = \prod_{i=1}^{d} \frac{1 + y_i x_i}{2}$. Sample random values $v_{y} \in \{-1, 1\}$ with probability $(0,5, 0.5)$ independently for each $y \in \{-1, 1\}^d$, the random hypercube polynomial function is $f(x) = \sum_{y \in \{-1, 1\}^d} v_y I_y(x)$.

For the random polynomial (random hypercube) functions, we use $d = 8$ and $D = 4$ in the this section and provide more results for other parameter settings in the appendix (for example, see Section~\ref{sec:manifold-exps} for when when the target polynomial functions concentrate on a low-dimensional subspace).

 

\subsection{Results} 

\mypar{MSE for random functions.} Figures \ref{fig:sparse_poly} and \ref{fig:sparse_hypercube} show the scaling behavior of the $\DSM$ and LSH models for a random polynomial function and  hypercube function (lower is better). Sparsity helps for the $\DSM$ and LSH models, both achieving better quality than dense models using the same number of activated units. In Figure~\ref{fig:comparison}, we compare the $\DSM$/LSH models with the random hash sparse models, and we see random hash sparse models underperform dense models, suggesting data-dependent sparsity mechanisms (such as $\DSM$/LSH) are effective ways to utilize sparsity.

\mypar{FLOPs.} To further qualify the efficiency gain of sparse models, we compare the MSE at the same FLOPs for sparse/dense models in Table~\ref{tab:flops}. The first column is the \# FLOPs for the dense model; models in the 3rd and 4th columns use same \# FLOPs but have more parameters (only 50\% or 25\% active). DSM uses only 18k FLOPs and gets smaller MSE than dense model with 73k FLOPs.

\begin{table}[h!]
    \centering
    \vspace{-0.05in}
    \begin{tabular}{|c|c|c|c|} \hline
    FLOPs & eval MSE (dense) & eval MSE (DSM 50\% sparsity) &  eval MSE (DSM 25\% sparsity)\\ \hline
    18432 & 0.01015	& 0.01014 &	{\bf 0.009655}\\ \hline
    36864 &	0.01009	& 0.007438 & {\bf 0.005054}\\ \hline
    73728 &	0.01046 & 0.006115	& {\bf 0.001799}\\ \hline
    \end{tabular}
    \caption{FLOPs and evaluation Mean Squared Error (eval MSE).}
    \vspace{-0.1in}
    \label{tab:flops}
\end{table}

\begin{figure}[h!]
  \centering
  \begin{subfigure}[b]{0.5\linewidth}
    \centering
    \includegraphics[width=\textwidth]{figs/dsm_scaling_sc.pdf}
    % \caption{DSM}
    \vspace{-0.15in}
    \label{fig:sparse_poly_a}
  \end{subfigure}%
  \begin{subfigure}[b]{0.5\linewidth}
    \centering
    \includegraphics[width=\textwidth]{figs/lsh_scaling_sc.pdf}
    %\caption{Hash vs Sparse}
    \vspace{-0.15in}
    \label{fig:sparse_poly_b}
  \end{subfigure}
  \caption{Scaling behavior of $\DSM$ and LSH models compared with dense models for a degree $4$ random polynomial with input dimension $8$: (a) $\DSM$ outperforms dense model at the same number of activated units and quality improves as total width increases; (b) LSH model outperforms dense model when number of buckets is large ($\geq 2048$) and quality improves as number of buckets increase.}
   \label{fig:sparse_poly}
   \vspace{-0.1in}
\end{figure}
\begin{figure}[h!]
  \centering
  \begin{subfigure}[b]{0.5\linewidth}
    \centering
    \includegraphics[width=\textwidth]{figs/hypercube_dsm_scaling_sc.pdf}
    % \caption{Sparse vs Dense}
    \vspace{-0.15in}
    \label{fig:sparse_cube_a}
  \end{subfigure}%
  \begin{subfigure}[b]{0.5\linewidth}
    \centering
    \includegraphics[width=\textwidth]{figs/hypercube_lsh_scaling_sc.pdf}
    % \caption{Hash vs Sparse}
    \vspace{-0.15in}
    \label{fig:sparse_cube_b}
  \end{subfigure}
  \caption{Scaling behavior of $\DSM$ and LSH models compared with dense models for a random hypercube function with input dimension $8$. Both $\DSM$ and LSH models outperform corresponding dense models with the same number of activated units (note: \# activ.~units $\leq$ width).}
   \label{fig:sparse_hypercube}
   \vspace{-0.1in}
\end{figure}



\mypar{CIFAR-10.} We also compare the scaling behavior of DSM and dense models on CIFAR-10~\cite{cifar}. The baseline model is a CNN with $3$ convolutional layers (followed by max-pooling), a dense layer with varying number of units, and a final dense layer that computes the logits (referred as CNN + dense). For the data-dependent sparse models, we use the same architecture, except we change the penultimate dense layer with a data-dependent sparse layer that choose the Top-$K$ activations (referred as CNN + DSM). Both models are trained with ADAM optimizer for $50$ epochs and evaluated on the test dataset for model accuracy with no data augmentation; see Figure~\ref{fig:cifar10} and Table~\ref{tab:cifar10} for the accuracy versus number of activated units. As with the synthetic datasets,  DSMs outperform dense models at the same number of activated units.

% \begin{figure}[h!]
%   \centering
%   \includegraphics[scale=0.35]{figs/cifar10_sparse_vs_dense_scaling_w_1024.pdf}
%   \caption{Scaling behavior of $\DSM$ compared with dense models on the CIFAR-10 dataset. Similar to Figure~\ref{fig:sparse_poly_a}, $\DSM$ outperforms dense models at the same number of activated units. }
%   \label{fig:cifar10}
%   \vspace{-0.1in}
% \end{figure}

% \begin{table}[h!]
%     \centering
%     \vspace{-0.225in}
%     \caption{CIFAR-10: Dense vs DSM eval accuracy at the same number of activated units}
%     \begin{tabular}{|c|c|c|c|} \hline
%     Activated units & dense & DSM, 50\% sparsity &  DSM, 25\% sparsity\\ \hline
%     256	& 69.79 & {\bf 70.74} & 69.8\\ \hline
%     512	& 70.79	 & 71.33 & {\bf 71.68}\\ \hline
%     \end{tabular}
%     \label{tab:cifar10}
% \end{table}
%  \vspace{-0.05in}
 
 
 
 \subsection{Discussion} 
 Our experimental results
 (e.g., Figures \ref{fig:sparse_poly},  \ref{fig:sparse_hypercube}, and \ref{fig:comparison}) show that sparsely activated models can efficiently approximate both random polynomials and random hypercube functions. Intuitively, the $\DSM$ and $\LSH$ models employ the sparsity as a way to partition the space into nearby input points.  Then, because the target function is Lipschitz, it is easy to provide to local approximation tailored to the specific sub-region of input space. On the other hand, the uniform random hash function performs poorly for these tasks precisely because it does not capture the local smoothness of the target function.
 
 On CIFAR-10, we also see that the $\DSM$ model performs comparably or better than the dense network. In particular,  Figure~\ref{fig:cifar10} shows that the ``CNN + DSM'' approach with total width 1024 improves upon or matches the dense model. In this case, the sparse activation allows the network to classify well while using only a fraction of the number of FLOPs. In Table~\ref{tab:cifar10}, we see that $\DSM$ model outperforms the dense model when we control for the number of activated units in the comparison.
 
 % {\color{red} TODO summarize that we've learned that sparse networks work well.}

% {\color{red} TODO discuss the differences in LSH vs DSM and argue that they are good models.} Address in the experimental set-up section.


\mypar{Limitations.} Our experiments focus on small datasets and 2-layer networks as a way to align with our theoretical results. Prior work on sparsely activated networks has shown success for large-scale NLP and vision tasks. Our experiments complement previous results and justify the $\DSM$ and $\LSH$ models by showing their ability to approximate Lipschitz functions (consistent with our theorems). It would be good to further evaluate the $\DSM$ and $\LSH$ models for large-scale tasks, for example, by using them as inspiration for routing functions in MoE vision transformers, such as V-MoE~\cite{riquelme2021scaling}. It would be interesting to evaluate on larger datasets, such as ImageNet as well. We experimented with a handful of hyperparameter settings, but a full search may lead to different relative behavior between the models (similarly, we only evaluated a few parameter settings for the random functions and the synthetic data generation, which is far from exhaustive).


\begin{figure}[t!]
  \centering
  \begin{subfigure}[b]{0.5\linewidth}
    \centering
    \includegraphics[width=\textwidth]{figs/lsh_dsm_hash_sc.pdf}
    \caption{random polynomial}
    \label{fig:sparse_poly_a_hash}
  \end{subfigure}%
  \begin{subfigure}[b]{0.5\linewidth}
    \centering
    \includegraphics[width=\textwidth]{figs/hypercube_lsh_dsm_hash_sc.pdf}
    \caption{random hypercube function}
    \label{fig:sparse_poly_b_hash}
  \end{subfigure}
  \caption{Scaling behavior of dense, random hash, $\DSM$, and LSH models. $\DSM$ and LSH models outperform dense models, while random hash models underperform dense models with the same number of activated units.}
   \label{fig:comparison}
   \vspace{-0.1in}
\end{figure}

 \begin{figure}[t]
\begin{floatrow}
\ffigbox{%
  \includegraphics[scale=0.25]{figs/cifar10_sparse_vs_dense_scaling_w_1024.pdf}%
}{%
  \caption{Scaling behavior of $\DSM$ compared with dense models on the CIFAR-10 dataset. Similar to Figure~\ref{fig:sparse_poly_a_hash}, $\DSM$ outperforms dense models at the same number of activated units. }%
  \label{fig:cifar10}
}
\capbtabbox{%
 \begin{tabular}{|c|c|c|} \hline
    Model \textbackslash \  \# activated units & 256 &  512 \\ \hline
    Dense	& 69.79 & 70.79 \\ \hline
    $\DSM$ (50\% sparse)	& {\bf 70.74}	 & 71.33 \\ \hline
    $\DSM$ (25\% sparse)	& 69.8	 & {\bf 71.68} \\ \hline
 \end{tabular}
}{%
  \caption{CIFAR-10 test accuracy for dense/$\DSM$ models with the same number of activated units. While not strictly monotonic, wider and sparser models outperform narrow and dense ones.}%
  \label{tab:cifar10}
}
\end{floatrow}
\end{figure}


% \begin{figure}[h!]
%   \centering
%   \includegraphics[scale=0.35]{figs/sparse_vs_dense_scaling_sc.pdf}
%   \caption{Sparse vs Dense scaling behavior for the random polynomial function.}
%   \label{fig:sparse_poly}
%   \vspace{-0.1in}
% \end{figure}
% \begin{figure}[h!]
%   \centering
%   \includegraphics[scale=0.35]{figs/hypercube_sparse_vs_dense_scaling_sc.pdf}
%   \caption{Sparse vs Dense scaling behavior for the random hypercube function.}
%   \label{fig:sparse_hypercube}
%   \vspace{-0.1in}
% \end{figure}

% \subsubsection{Comparison with random hash based sparsity}
% \begin{figure}[h!]
%   \centering
%   \includegraphics[scale=0.35]{figs/hash_vs_sparse_scaling_sc.pdf}
%   \caption{Hash vs Sparse vs Dense scaling behavior for the random polynomial function.}
%   \label{fig:hash_poly}
%   \vspace{-0.1in}
% \end{figure}
% \begin{figure}[h!]
%   \centering
%   \includegraphics[scale=0.35]{figs/hypercube_hash_vs_sparse_scaling_sc.pdf}
%   \caption{Hash vs Sparse vs Dense scaling behavior for the random hypercube function.}
%   \label{fig:hash_hypercube}
%   \vspace{-0.1in}
% \end{figure}





==> Hybrid Sparsity (arxiv)/intro.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Introduction}
\label{sec:intro}

Overparameterized neural networks continue to yield performance gains as their sizes increase. This trend has been most prominent with large Transformer based language models \cite{brown2020language, devlin2018bert,raffel2019exploring}. However, using large, dense networks makes training and inference very expensive, and computing a forward pass may require trillions of floating point operations (FLOPs). It is an active area of research to improve the scalability and efficiency without decreasing the expressiveness or quality of the models. 

One way to achieve this goal is to only activate part of the network at a time. For example, the Mixture of Experts (MoE) paradigm~\cite{jordan1994hierarchical,shazeer2017outrageously} uses a two-step approach. First, each input is mapped to a certain subnetwork, known as an expert. Then, upon receiving this input, only this particular subnetwork performs inference, leading to a smaller number of operations compared to the total number of parameters across all experts. Some variations of this idea map parts of an input (called tokens) individually to different experts. Another well-studied generalization is to map an input to a group of subnetworks and aggregate their output in a weighted manner. Switch Transformers~\cite{fedus2021switch} successfully use a refined version of the MoE idea, where the input may be the embedding of a token or part of a hidden layer's output. Researchers have investigated many ways to perform the mapping, such as Scaling Transformers~\cite{jaszczur2021sparse} or using pseudo-random hash functions~\cite{roller2021hash}. In all cases, sparsity occurs in the network because after the input is mapped to the subnetwork, only this subset of neurons needs to be activated. Moreover, the computation of the mapping function, sometimes referred to as a `routing' function, takes significantly less time than the computation across all experts.

The success of these approaches is surprising. Restricting to a subnetwork could instead {\em reduce} the expressive power and the quality of the model. However, the guiding wisdom seems to be that it suffices to maximize the number of parameters while ensuring computational efficiency. Not all parameters of a network are required for the model to make its prediction for any given example. 
\rebut{Our goal is to provide a theoretical explanation for the power of sparse models on concrete examples.}

%Our goal is to analyze the approximation power of sparse models. 

% One challenge is that many of the transformer studies use large networks with many complex parts, and measure the performance in terms of \emph{perplexity} for language tasks~\cite{roller2021hash}. In general, it is hard to reason about large networks in entirety or about the task of optimizing the perplexity objective. Instead, we restrict our attention to networks with \emph{one} sparsely activated layer with a regression objective (i.e., mean squared error). Our motivation is to provide a way to zoom into the expressiveness of a single sparsely activated layer. We imagine this as one part of a larger network, where this component is responsible for learning a $d$-dimensional function.

\paragraph{Our Results.}
Our first contribution is a formal model of networks that have one or more sparsely activated layers. These sparse layers are data dependent: the subset of network activations and their weight coefficients depend on the input. We formally show that our model captures popular architectures (e.g., Switch and Scaling Transformers) by simulating the sparse layers in these models.

We next prove that \rebut{the above class of sparsely activated models} can learn a large class of functions \rebut{more efficiently than dense models}.
\rebut{As our main proof technique, we introduce a new routing function, based on locality sensitive hashing (LSH), that allows us to theoretically analyze sparsely activated layers in a network.}
%One of our main techniques is to use locality sensitive hashing (LSH) to determine the sparse layer. 
LSH maps points in a metric space (e.g., $\mathbb{R}^d$) to `buckets' such that nearby points map to same bucket. The total number of buckets used by a LSH function is referred to as the size of the hash table.
\rebut{Prior work has already identified many routing functions that work well in practice. We do not aim to compete with these highly-optimized methods, but rather we aim to use LSH-based routing as a way to reason about the approximation ability of sparse networks.}

In Theorem~\ref{thm:main-lipschitz-lsh-ub}, we show that LSH-based sparse models can approximate real-valued Lipschitz functions in $\mathbb{R}^d$. Although real data often lives in high dimensions, the underlying manifold where the inputs are supported is often assumed to be low-dimensional (e.g. the manifold of natural images vs $\mathbb{R}^{224 \times 224}$ for a $224\times 224$ image). We model this by assuming that our inputs lie in a $k$-dimensional manifold within $\mathbb{R}^d$. To get $\epsilon$ approximation error, we need an LSH table of size approximately $O((\sqrt{dk}/\epsilon)^k)$ but a forward pass only requires time $O(dk\log(1/\epsilon))$ as only one of the $O((\sqrt{dk}/\epsilon)^k)$ non-empty buckets are accessed for any given example.

% {\color{red} TODO update this with the new lower bound}
In Theorem~\ref{thm:dense-lb}, we complement our upper bounds by proving a lower bound of $\Omega((2\sqrt{d}/\epsilon)^k)$ on the size needed for both dense and sparse models (when points live in $k$ dimensions). This also transforms into a lower bound on the number of samples required to learn these functions using a dense model. This lower bound implies that a forward pass on a dense model takes time $\Omega(d(2/\sqrt{k}\epsilon)^k)$, which is exponentially worse than the time taken by the sparse model.
Altogether, we show that for the general class of Lipschitz functions, sparsely activated layers are as expressive as dense layers, while performing significantly fewer floating point operations (FLOPs) per example.

% {\color{red} We also strengthen our lower bound construction in Theorem~\ref{thm:dense-lb} to hold for not only Lipschitz functions but also analytic functions. These are smooth functions that are differentiable everywhere. Theorem~\ref{thm:dense-lb-analytical} provides this stronger construction.}

\rebut{To support our theory, we perform experiments in Section~\ref{sec:experiments} on approximating Lipschitz functions with sparse networks.}
%We perform experiments in Section~\ref{sec:experiments} that investigate the relative power of various models. 
\rebut{We identify several synthetic datasets where models with data-dependent sparse layers outperform dense models of the same size. Moreover, we achieve these results with relatively small networks. This provides a few minimum working examples of when sparsity is beneficial. 
Our results complement the existing work that has already shown the success of very large MoE models on real-world NLP and vision tasks~\cite{fedus2021switch, jaszczur2021sparse, riquelme2021scaling}.}
%Hence, we shed new light on MoE-based techniques, and we 
%While this does not explain the success of very large MoE models, it does provide a minimum working example of when sparsity can be beneficial. 
Our experiments also generalize the intuition from Figure \ref{fig:1d_lsh}, where the model outputs a different constant value for each bucket.
%By studying scaling behaviors as the model size grows, we demonstrate models with data-dependent sparse layers outperform dense models of the same size. 
%The results verify our intuition as suggested by the one dimensional example shown in Figure \ref{fig:1d_lsh}, in which a locality sensitive hashing (LSH) layer (a form of data-dependent sparsity) allows the model to learn simple, constant functions in each bucket.
A puzzling empirical result was observed in \cite{roller2021hash} where a pseudo-random uniform hash function is used to route input tokens to experts. Intuitively, this might map very nearby or similar points to distinct experts, leading to a potentially non-smooth behavior. 
\rebut{We show that on our synthetic, Lipschitz datasets, the $\LSH$ model outperforms uniform random hashing, which further corroborates our theory.}
%We also investigate the uniform hash router by comparing our models against it. We find that, in contrast to \cite{roller2021hash}, the $\LSH$ model is more effective than uniform random hashing for learning Lipschitz functions.


% former one utilizes sparsity more effectively.

% \begin{figure}[h!]
%   \centering
%   \includegraphics[scale=0.3]{figs/1d_lsh.pdf}
%   \vspace{-0.2in}
%   \caption{Learning a polynomial function with a LSH model using $16$ hash buckets. Dashed curve is the target function graph, piecewise constant curve is the learned LSH model output, and different LSH buckets are indicated by different colors. Note neighboring points are hashed to the same bucket, in which a simple constant can be learned to approximate target function values.}
%   \label{fig:1d_lsh}
% \end{figure}
\begin{figure}[h!]
  \centering
  \begin{subfigure}[b]{0.5\linewidth}
    \centering
    \includegraphics[width=\textwidth]{figs/1d_lsh.pdf}
    \caption{1D example}
    \label{fig:1d_lsh}
  \end{subfigure}%
  \begin{subfigure}[b]{0.5\linewidth}
    \centering
    \includegraphics[width=\textwidth]{figs/dsm_scaling_sc.pdf}
    \caption{sparse/dense scaling behavior}
    \label{fig:sparse_vs_dense}
  \end{subfigure}
  \vspace{-0.2in}
  \caption{Learning polynomial functions with data-dependent sparse models: (a) Dashed curve is the target function graph, piecewise constant curve is the learned LSH model output, and different LSH buckets are indicated by different colors. Note neighboring points are hashed to the same bucket, where a simple constant can be learned to approximate target function values; (b) Scaling behavior of data-dependent sparse models (DSM) versus dense models, in which sparse models outperform dense models of the same size, see Section \ref{sec:prelims} and Section \ref{sec:experiments} for details.}
  \label{fig:intro_expt}
\end{figure}

\paragraph{Related Work.}
\label{sec:relatedwork}
Sparsely activated networks have had enormous empirical success~\cite{allingham2021sparse, artetxe2021efficient,du2021glam, kim2020fastformers, nie2021dense, riquelme2021scaling, shazeer2017outrageously, wang2021ernie}. 
The Switch Transformer~\cite{fedus2021switch} is one of the first major, contemporary applications of the sparsely activated layers. Follow-up works such as Scaling Transformers~\cite{jaszczur2021sparse} and other hash functions~\cite{roller2021hash} aim to improve the sparse layers. These papers build upon seminal MoE works~\cite{jacobs1995methods, jacobs1991adaptive, jordan1994hierarchical}, and other uses of the MoE paradigm~\cite{lepikhin2021gshard,shazeer2018mesh-tensorflow}.  
% While prior work on sparse transformers considers language tasks,
There has been work on using statistical mechanics to analyze the generalization of MoE models~\cite{kang1996statistical}. However, to the best of our knowledge, there is no systematic theoretical study of modern sparsely activated networks. 
% We aim to bridge this gap.

The above work on dynamic sparsity builds on previous \emph{static} sparsity efforts, e.g., weight quantization~\cite{li2020train}, dropout~\cite{srivastava2014dropout}, and pruning (see the survey~\cite{hoefler2021sparsity} and references). Static sparsity means that the subnetwork activation does not change in a data-dependent way. The focus is on generalization and compression, instead of achieving fast inference time with a huge number of parameters. 

% This has been observed to be less effective for large-scale learning tasks (e.g., question answering, summarization, translation).
% that are common in NLP.
% 

Our work builds on locality sensitive hashing (LSH), a well-studied technique for approximate nearest neighbor search (see the survey~\cite{andoni2018approximate} or the book~\cite{har2011geometric} and references therein for LSH background). A seminal and popular LSH family uses random hyperplanes to partition the space~\cite{andoni2015practical, charikar2002similarity}. Another option is to use balls centered at lattice points, which works well for $\ell_2$ distance~\cite{andoni2006near}. We use these ideas to design sparse networks. For uses of LSH in deep learning, sketch-based memory improves network capacity~\cite{ghazi2019recursive, panigrahy2021sketch}. Other empirical work uses LSH to improve dense network training time or memory~\cite{chen2020mongoose, chen2015compressing, rae2016scaling}. Our work differs from the prior studies because we implement the LSH-based approach with sparsely activated networks, with the goal of reducing inference time and achieving low regression error. LSH-based sparsity may be most relevant for vision transformers~\cite{khan2021transformers, riquelme2021scaling, wu2020visual}, using distance metrics and routing functions tailored to images, or for time series analysis~\cite{wen2022transformers}.

% {\color{red} Some of our results focus on a restricted training set-up, where only the sparse layer depends on the target function and the bottom layer is randomly initialized. Analyzing the approximation power of fully trainable networks is challenging even at depth 2; results are known for simple functions, e.g., parities~\cite{daniely2020learning} or at very large widths~\cite{jacot2018neural, allen2019convergence}. We also speculate on possible improvements from having full trainability for future work.}

% Another type of sparsity is Drop-out~\cite{srivastava2014dropout}, but this does not improve the computation time of inference.



% Although the MoE idea has existed for a while, previous efforts did not succeed to scaling to real-world network sizes~\cite{lepikhin2021gshard,jordan1994hierarchical, shazeer2017outrageously,shazeer2018mesh-tensorflow}. 

% One way is to do something data-dependent, like dropout, which does not reduce inference time. Another way is to remove connections after training, but this leads to a single sparse network, and this is known to work poorly for NLP tasks. Instead, the MoE framework allows you to choose among different networks, without losing information.


%%%% old text 


% One recent approach which has seen success recently is an approach based on Mixture of Experts (MoE) which scales up the number of parameters without scaling up the compute of a forward pass. Such scaling when done carefully has lead to improved quality at significantly lower inference costs.
% More efforts underway (Pathways) to decouple inference costs from total size of a model. These are based on the following hypothesis: 
% In this work, we aim to develop a theoretical understanding behind the efficacy of such MoE models.
% We focus on simpler scenarios with shallow networks where we can provably show the gains of a hybrid sparse structure over a dense one. Although in practice, networks are deep the same principles we outline here apply.
% \nishanth{one potential reviewer complaint on our model could be that it is shallow. should address this?}


==> Hybrid Sparsity (arxiv)/lsh_to_dsm.tex <==
\section{Simulating Models with DSM}
\label{sec:model-results}
We formally justify the $\DSM(d,s,t)$ model by simulating other models using it.
We start with simple examples (interpolation, $k$ nearest neighbor ($k$-NN) regression, and Top-$K$), then move on to transformers and the LSH model. For the simple examples, we only need one hidden layer, where $\phi(x) = \sigma(Bx)$ for a matrix $B \in \mathbb{R}^{t\times d}$ and non-linearity $\sigma$.
% We focus on the sparse vector $A^x$, and assume that the matrix $B$ and non-linearity $\sigma$ vary per the application. 
% \subsection{Interpolation and $k$-NN}
% To gain intuition, consider  $\DSM$ on two examples: interpolation and $k$ nearest neighbor ($k$-NN) regression. 

\mypar{Interpolation.} We show how to compute $f$ at $t$ points $x_1,\ldots,x_t$. We only need sparsity $s = 1$ and \rebut{$\sigma$ is simply the identity function.}
We set $A_i = f(x_i) / \langle b_i, x_i \rangle$, where $b_i$ is the $i$th row of $B$.
Further, we let $\mathsf{mask}(x_i)$ have a one in the $i$th position and zeroes elsewhere. Then, we define 
$g(x_i) = (A \circ \mathsf{mask}(x_i))Bx_i = f(x_i)$, which computes $f$ at the $t$ input points. 

\mypar{Sparse networks perform $k$-NN regression}. 
We sketch how the $\DSM(d,k,n)$ model can simulate $k$-NN with $g(x) = (A\circ \mathsf{mask}(x)) \sigma(B x)$, when the dataset contains vectors with unit $\ell_2$ norm.Let the rows of $B$ be a set of $n$ unit vectors $b_1,\ldots,b_n \in \mathbb{R}^d$. For the target function~$f$, let $A = \frac{1}{k}(f(b_1),\ldots,f(b_n))$.
Define $\sigma(B x)$ to have ones in the top $k$ largest values in $B x$ and zeroes elsewhere. For a unit vector $x$, these $k$ positions correspond to the $k$ largest inner products $\langle x, b_i \rangle$. Since 
$\|x - b_i\|_2 = 2 - 2\langle x, b_i \rangle$,  the non-zero positions in $\sigma(B x)$ encode the $k$ nearest neighbors of $x$ in $\{b_1,\ldots,b_n\}$.
Thus, $g(x)$ computes the average of $f$ at these $k$ points, which is exactly $k$-NN regression. Moreover, only $k$ entries of $A$ are used for any input, since $\sigma(Bx)$ is $k$-sparse; however, computing $\sigma(Bx)$ takes $O(nd)$ time.
While there is no computational advantage from the sparsity in this case, the fact that $\DSM$ can simulate $k$-NN indicates the power of the model.
% This view indicates the power of the $\DSM$ model, partially explaining why sparse layers work well in practice.

\mypar{Simulating Top-$K$ routing.} For an integer $K \in \mathbb{N}^+$, certain MoE models choose the $K$ largest activations to enforce sparsity; in practice, $K \in \{1,2\}$ is common~\cite{riquelme2021scaling}. We use $\mathsf{mask}(x)$ with $\|\mathsf{mask}(x)\|_0 = K$ as the indicator for the $K$ largest values of $Bx$. Then, $\sigma$ is the identity, and $g(x) = (A\circ \mathsf{mask}(x)) B x$ applies $A$ to the top $K$ entries of $Bx$.

\subsection{Simulating transformer models with $\DSM$}
Real-world networks have many hidden layers and multiple sparse layers. For concreteness, we describe how to simulate a sparsely activated final layer. As mentioned above, we can compose functions in the $\DSM$ model to simulate multiple sparse layers.
% 2-layer models, that capture one of the sparse layers that comes after one of the dense layers.

\mypar{Switch Transformers~\cite{fedus2021switch}.} The sparse activations in transformers depend on
a \emph{routing function} $R: \mathbb{R}^d \to \{1,\ldots, L\}$, where $R(x)$ specifies the subnetwork that is activated (for work on the best choice of $R$, see e.g.,~\cite{roller2021hash}). To put this under the $\DSM(d,s,t)$ model, consider a set of trainable matrices $A_1,\ldots, A_L \in \mathbb{R}^{1 \times s}$, where the total width is $t = s \cdot L$. On input $x$, we think of $A^x$ as a $1 \times t$ matrix with $s$ non-zero entries equal to $A_{R(x)}$. In other words, $A$ is the concatenation of $A_1,\ldots, A_L$, and $\mathsf{mask}(x)$ is non-zero on the positions corresponding to $A_{R(x)}$.
% For sparsity, we enforce that each $A_i$ has at most $s$ non-zero entries. 

\mypar{Scaling Transformers~\cite{jaszczur2021sparse}.} 
The key difference between Switch and Scaling transformers is that the latter imposes a block structure on the sparsity pattern. Let $t$ be the width, and let $s$ be the number of blocks (each of size $t' = t/s$). Scaling Transformers use only one activation in each of the $s$ blocks. In the $\DSM(d,s,t)$ model, we capture this with $A^x$ as follows.  Let $e_i \in \{0,1\}^{t'}$ denote the standard basis vector (i.e., one-hot encoding of $i \in [t'])$. The sparsity pattern is specified by indices $(i_1,\ldots, i_s)$. Then, $A^x = (\alpha_1 e_{i_1},\ldots, \alpha_b e_{i_s})$ for scalars $\alpha_1,\ldots, \alpha_s \in \mathbb{R}$.

\subsection{Simulating the $\LSH$ model using $\DSM$}

We explain how to represent the $\LSH$ model using the $\DSM$ model. The key aspect is that $A^x$ depends on the LSH buckets that contain $x$, where we have $s$ non-zero weights for the $s$ buckets that contain each input. This resembles the Scaling Transformer, where we use the LSH buckets to define routing function.
In the $\LSH(d, s, m, \Delta)$ model, there are $s$ sets of $m$ hash functions, leading to $s \cdot 2^m$ hash buckets. We use width $t = s \cdot 2^m$ for the $\DSM(d,s,t)$ network. The entries of $A^x$ are in one-to-one mapping with the buckets, where only $s$ entries will be non-zero depending on the $s$ buckets that $x$ hashes to, that is, the values $(h^i_1(x),\ldots, h^i_m(x)) \in \{-1,1\}^m$ for $i = 1,2,\ldots, s$. 



We now determine the values of these $s$ non-zero entries. We store a degree $\Delta$ polynomial $\hat g(x) :\mathbb{R}^d \to \mathbb{R}$ associated with each bucket. For our upper bounds, we only need degree $\Delta=0$, but we mention the general case for completeness. If $\Delta=0$, then $\hat g$ is simply a constant $\alpha$ depending on the bucket. 
An input $x$ hashes to $s$ buckets, associated with $s$ scalars $(\alpha_1,\ldots, \alpha_s)$. To form $A^x$, set $s$ entries to the $\alpha_i$ values, with positions corresponding to the buckets. For degree $\Delta \geq 1$, we store coefficients of the polynomials $\hat g$, leading to more parameters. Section~\ref{sec:sparse-random-functions} describes how to use LSH-based sparse networks to approximate Lipschitz functions.

\mypar{Computing and storing the LSH buckets.} Determining the non-zero positions in $A^x$ only requires $O(sm)$ hash computations, each taking $O(d)$ time with standard LSH families (e.g., hyperplane LSH). 
% Using many known LSH families, we can ensure that computing $A^x$ only takes $O(sd)$ time.
We often take $m$ to be a large constant. Thus, the total number of operations to compute a forward pass in the network $O(smd) \approx O(sd)$.  The variable $m$ above determines the total number of distinct buckets we will have ($2^m$). For an $n$ point dataset, $m = O(\log n)$ is a realistic setting in theory. Therefore, $2^m = \mathrm{poly}(n)$ is often a reasonable size for the hash table and moreover the dense model requires width $O(2^m)$ as well. In practice, the number of experts is usually 32--128~\cite{fedus2021switch, riquelme2021scaling}.
The hash function typically adds very few parameters. For example, to hash $d$ dimensional data into $2^m$ buckets, LSH requires $O(md)$ bits and takes $O(md)$ time as well. In summary, the LSH computation does not asymptotically increase the number of FLOPs for a forward pass in the network. We also later bound the number of non-empty LSH buckets. The memory to store the hash table is comparable to the number of samples required to learn the target function.

% \subsection{Further Model Questions}




% in a region. Let $\bar x$ be a representative point in this region (e.g, the center). 
% When $s=1$, we can choose a single index $i$ to be non-zero, and set $A_i^x = f(x) / \langle b_i, x \rangle$, where $b_i$ is the $i$th row of $B$. Then, we exactly have $g(x) = A^xBx = f(x)$. 
% To approximate $f$ outside of these $t$ points, we optimize the weights in $A$. In general, we use a $\mathsf{mask}$ function based on LSH, and we consider $s>1$.
% Here, the approximation may work well, but we are ignoring the information provided by $\langle b_i, x \rangle$. For $s>1$, the optimal setting of weights in $A^x$ is not immediate at all, and requires training to learn. 

% \mypar{Training the lower layer.}
% Representation-wise, if allow training of the lower layer (the matrix $B$ in the $\DSM$ model), we can express more functions. This layer defines a projection of $x$ into the representation $Bx$. Then, we perform a sparse computation in this space. With more layers, we can capture non-linear transformations, such as to manifolds. For the $k$-NN example above, 
% the sparse activation pattern changes over time (i.e., the $k$ neighbors change). The top layer computes the $k$-NN regression in the representation space. 
% We leave these as interesting future directions.

==> Hybrid Sparsity (arxiv)/neurips_checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}



\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{See sections~\ref{sec:theory-apdx} and~\ref{sec:experiments} }
  \item Did you describe the limitations of your work?
    \answerYes{See Sec.~\ref{sec:sparse-random-functions} and \ref{sec:conclusion}.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{Our work is primarily theoretical, without targeted applications.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{See Section~\ref{sec:sparse-random-functions} and Sections~\ref{sec:manifolds-apdx} and \ref{sec:theory-apdx} of the Appendix.}
        \item Did you include complete proofs of all theoretical results?
    \answerYes{See Section~\ref{sec:sparse-random-functions} and Sections~\ref{sec:manifolds-apdx} and \ref{sec:theory-apdx} of the Appendix.}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
\answerYes{We include details to reproduce all datasets and experiments.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
        \answerYes{Details about our experiments are in Section~\ref{sec:experiments} and Section \ref{sec:experimental-details-apdx} of the Appendix.}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNo{}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerNo{}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{See Section~\ref{sec:experiments}}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
  \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> Hybrid Sparsity (arxiv)/parities.tex <==
\section{Properties of Learning Parities Problem}
Learning parity on $k$ bits of a $d$-dimensional input has a polynomial sample complexity. Parity without noise is easy both sample complexity wise and computationally. 
Parity with noise is hard to learn efficiently. But it can be learnt with a with linearly many samples and an exponential time algorithm as long as $k < d/\log d (d^k < 2^d)$. (i.e. it is PAC learnable but not PAC learnable efficiently)
BKW is an algorithm for LPN which uses super-polynomial number of samples to learn parities in sub-exponential time.

An observation on the Learning Parities paper \cite{daniely2020learning}:
Their upper bound for 2-layer trainable NN is stylized to work for parity function which is a single monomial once we find the right subset $A$. If we choose a linear combination of parities over all possible $A$ of size $k$ then their upper bound won’t hold.

Questions:
1. Focusing on the parities example, and allowing ourself exponential width in $k$, what is the right time complexity for learning for both dense linear layer vs sparse linear layer?
2. Focusing on parities example again, and allowing a trainable bottom layer what is the time-space tradeoff curve for both dense top layer vs sparse top layer?

==> Hybrid Sparsity (arxiv)/preamble.tex <==
\usepackage{PRIMEarxiv}
\usepackage{fancyhdr}       % header
\usepackage{graphicx}       % graphics
% \usepackage{natbib}
\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{hyperref}       % hyperlinks
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
%  \usepackage{xcolor}         % colors
\usepackage[dvipsnames,svgnames,x11names,hyperref, enumerate]{xcolor}
\definecolor{blueish}{HTML}{007F99}
\definecolor{purpleish}{HTML}{72177A}
\definecolor{grape}{HTML}{6f2da8}
\definecolor{magenta}{HTML}{c229a9}
\hypersetup{
	colorlinks,
	citecolor=purpleish,
	filecolor=red,
	linkcolor=blueish,
	urlcolor=Blue
}


% For theorems and such
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{mathtools}
\usepackage{amsthm}
\usepackage{caption}
\usepackage{subcaption}

% if you use cleveref..
\usepackage[capitalize,noabbrev]{cleveref}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% THEOREMS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{assumption}[theorem]{Assumption}
\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}


% Todonotes is useful during development; simply uncomment the next line
%    and comment out the line below the next line to turn off comments
%\usepackage[disable,textsize=tiny]{todonotes}
\usepackage[textsize=tiny]{todonotes}

\DeclareMathOperator*{\E}{\mathbb{E}}
\newcommand{\nishanth}[1]{{\color{purple}{Nishanth: #1}}}
\newcommand{\rina}[1]{{\color{blue}{Rina: #1}}}
\newcommand{\cyrus}[1]{{\color{green}{Cyrus: #1}}}

\newcommand{\sgn}{\mathop{\mathrm{sgn}}}
% \newcommand{\mypar}[1]{\smallskip \noindent \textbf{#1}}
\newcommand{\mypar}[1]{\noindent \textbf{#1}}
\newcommand{\DSM}{\mathsf{DSM}}
\newcommand{\LSH}{\mathsf{LSH}}
\newcommand{\eps}{\epsilon}

% The \author macro works with any number of authors. There are two commands
% used to separate the names and addresses of multiple authors: \And and \AND.
%
% Using \And between authors leaves it to LaTeX to determine where to break the
% lines. Using \AND forces a line break at that point. So, if LaTeX puts 3 of 4
% authors names on the first line, and the last on the second line, try using
% \AND instead of \And before the third author name.


\author{%
  Cenk Baykal \\
  Google Research \\
  \texttt{baykalc@google.com} \\
  % examples of more authors
  \And
  Nishanth Dikkala \\
  Google Research \\
  \texttt{nishanthd@google.com} \\
  \AND
  Rina Panigrahy \\
  Google Research \\
  \texttt{rinap@google.com} \\
  \And
  Cyrus Rashtchian \\
  Google Research \\
  \texttt{cyroid@google.com} \\
  \And
  Xin Wang \\
  Google Research \\
  \texttt{wanxin@google.com} \\
}

==> Hybrid Sparsity (arxiv)/prelims.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Preliminaries}
\label{sec:prelims}
Let $f:\mathbb{R}^d \to \mathbb{R}$ be a multivariate real-valued function that we want to learn with a neural network. We consider regression, and we aim to minimize the mean-squared error or the $\ell_{\infty}$ error.
For a function $f$ defined on a set $\Gamma$ and an estimator $\hat{f}_n$, we define
% $\|f-\hat{f}_n\|_{\infty}$ as
$\|f - \hat{f}_n\|_{\infty} = \sup_{x \in \Gamma} |f(x) - \hat{f}_n(x)|.$
% \begin{align}
%     \|f - \hat{f}_n\|_{\infty} = \sup_{x \in \Gamma} |f(x) - \hat{f}_n(x)|.
% \end{align}
For some results, we approximate $f$ on a subset $\mathcal{V} \subseteq \mathbb{R}^d$. For example, $\mathcal{V}$ may be the intersection of $[-1,1]^d$ and a $k$-dimensional subspace. We also consider the case when $f$ is $L$-Lipschitz, meaning that $|f(x) - f(x')| \leq L\cdot \|x-x'\|_2$ for all $x, x' \in \mathbb{R}^d$. We define $[n] = \{1,2,\ldots, n\}$.

\subsection{Data-Dependent Sparse Model}
% {\color{red} can we rephrase for deeper networks?? replace $B$ with a general function $\phi:\mathbb{R}^d \to \mathbb{R}^t$}

A dense neural network $g$ with a fully connected final layer can be expressed as $g(x) = A \cdot \phi(x)$ where $A \in \mathbb{R}^{1 \times t}$ is a matrix and $\phi: \mathbb{R}^{d} \to \mathbb{R}^t$ is a function (e.g., $\phi$ captures the representation learned up until the final layer). Here, $t$ is the width of the final layer and $d$ is the input dimensionality.

Our focus is on the types of networks captured by what we call the \emph{Data-Dependent Sparse Model ($\DSM$)}. 
This is a network with a sparsely activated final layer. Formally, let $t$ be the width, and let $s \leq t$ be a sparsity parameter. Then, we consider functions $g$ of the form
$g(x) = A^x \cdot \phi(x)$ where 
$A^x \in \mathbb{R}^{1 \times t}$ and $\phi: \mathbb{R}^{d} \to \mathbb{R}^t$. The crux of the model is the final layer. The sparsity comes from letting $A^x = A \circ \mathsf{mask}(x)$, where $\mathsf{mask}(x) \in \{0,1\}^{1 \times t}$ is an $s$-sparse indicator vector, and  ``$\circ$'' is the entry-wise product. The mask zeroes out certain positions, and $A$ contains the learned weights but no longer depends on~$x$. 
Intuitively, the $\mathsf{mask}$ is the ``routing function'' for the sparse activations. To do so, we define  $\mathsf{mask}(x) \circ \phi(x)$ to mean that we zero out element of the vector $\phi(x)$. Then, we have 
% the equivalence 
$$g(x) = (A \circ \mathsf{mask}(x)) \phi(x)  = A (\mathsf{mask}(x) \circ \phi(x)).$$ 
Under the above definitions, let $\DSM(d,s,t)$ be the set of functions $g = (A \circ \mathsf{mask}(x)) \cdot \phi(x)$. In what follows, we use $A^x$ as shorthand for $A \circ \mathsf{mask}(x)$.

% TODO address the time it takes to build the LSH table
% It is desirable to be able to determine $A^x$ efficiently. For example, if computing $\mathsf{mask}(x)$ takes $O(sd)$ time, then $g(x)$ only uses $O(sd)$ operations when we can efficiently restrict to these $s$ rows of $\phi(x)$. This is less than $O(td)$ when $s \ll t$. 

In the $\DSM$ model, we wish to understand the effect of sparsity on how well the network can approximate certain functions. It is important to allow the final layer $A^x \in \mathbb{R}^{1 \times t}$ to be data-dependent. The values in $A^x$ depend on the target function $f$, and we learn this from training data. 

Real-world transformers may have multiple sparse layers. To capture this, we can compose $\DSM$ functions. For example, two sparse layers comes from $g(x) = A \circ \mathsf{mask}_2(x) \circ \phi_2(\mathsf{mask}_1(x) \circ \phi_1(x))$.  For simplicity, we focus on a single sparse layer in what follows, which suffices for our main results.
% For some of our results, we make the simplifying assumption that the hidden layer $B \in \mathbb{R}^{t \times d}$ is \emph{not} trainable, but instead, it is a random matrix. This enables us to focus on the sparsity of $A^x$ without analyzing the training dynamics of the larger matrix $B$. We show later show theoretically and empirically that this restriction does not prohibit the network from fitting complicated functions.

\subsection{Hash-based Routing}

Prior sparse models compute hash functions of the input vector $x$ to determine $\mathsf{mask}$ and the network activations~\cite{roller2021hash}. 
Our main theorem uses this strategy, considering LSH families. LSH has the property that nearby points are more likely to end up in the same hash bucket than far away points. We can use LSH to define a general class of efficient regression functions. In Section~\ref{sec:model-results}, we prove that the $\DSM$ model captures popular sparse architectures and the following $\LSH$ model.

\mypar{$\LSH$ Model.} We review an $\LSH$ framework based on sign patterns. Let $h_1,\ldots, h_m:\mathbb{R}^d \to \{-1,1\}$ be $m$ distinct hash functions. Partition the space into $2^m$ buckets based on the $m$ sign patterns $z_x = (h_1(x),\ldots,h_m(x))$ over all $x \in \mathbb{R}^d$. 
Then, for each $z \in \{-1,1\}^m$, we can specify a function $\hat g_{z}(x)$, where the goal is for $g_z$ to approximate the target function $f$ in the part of space associated with $z$ (i.e., points $x$ that have pattern $z$ under $h_1,\ldots, h_m$). More generally, we can allow $s$ sets of such hash functions $(h^i_1,\ldots, h^i_m)$, and $s$ sets of these approximation functions $(\hat g^1_{z^1},\ldots, \hat g^s_{z^s})$ for $i = 1,\ldots, s$. On input $x$, we compute the sign patterns $z^1, \ldots, z^s$ and output $g(x) = \sum_{i=1}^s \alpha_i \hat g^i_{z^i}(x)$. Further, we can restrict each $\hat g^i_z$ to be a degree $\Delta \geq 0$ polynomial. For a fixed LSH family of possible hash functions, we let $\LSH(d, s, m, \Delta)$ denote this class of functions. In many cases, we only need $\hat g^i_z$ to be a constant function, i.e., $\Delta=0$, and we shorten this as $\LSH(d, s, m, 0) := \LSH(d, s, m)$. Our goal is to understand the trade-offs of the ``memory'' parameter $m$ and the ``sparsity'' amount $s$ that we need to approximate large classes of $d$-dimensional functions (i.e., $L$-Lipschitz functions supported on a $k$-dimensional manifold).

\mypar{Euclidean $\LSH$ Model \cite{datar2004locality}.} This is a popular LSH family for points in $\mathbb{R}^d$. In this case, each hash function outputs an integer (instead of $\pm 1$ above). Each bucket in this model is defined by a set of hyperplane inequalities. There are two parameters $(D,\epsilon)$. We sample $D$ random directions $a_1, \ldots, a_D$ where each coordinate of each $a_i$ is an independent normal variable. In addition we sample $b_i \sim \mathrm{Unif}[0,\epsilon]$ independently for $i \in [D]$.  For a point $x \in \mathbb{R}^d$, we compute an index into a bucket via a function $h_i : \mathbb{R}^d \to \mathbb{Z}$ defined as
% \begin{align}
% $
%     \left(\left\lfloor \frac{a_i^\top x + b_i}{\epsilon} \right\rfloor \right)_{i=1}^D.
% $
$$
    h_i(x) = \left\lfloor \frac{a_i^\top x + b_i}{\epsilon} \right\rfloor. 
$$ Here, the index $i$ ranges over $i \in [D]$, leading to a vector of $D$ integers. %\cnote{If each hash function corresponds to $a_i$, $b_i$, does that mean the number of hash functions $m$ is equal to $D$?}
%\nishanth{Yes, this can be thought of as a composition of $D$ hash functions of size $T$ or a single function of table size $2^DT$}

% \end{align}




% Let $h_1,\ldots, h_s:\mathbb{R}^d \to \{-1,1\}$ be $s$ distinct functions (e.g., $s$ random hyperplanes). We can partition the space into $2^s$ buckets based on the sign patterns $z_x = (h_1(x),\ldots,h_s(x))$ over all $x \in \mathbb{R}^d$. For each of these $2^s$ buckets, we can learn a linear function $\hat g_{z_x}(x)$ that approximates our target function $f$ in this part of the space. Then, we can approximate $f(x)$ with $g(x) = \hat g_{z_x}(x)$, which only depends on the linear function $g_{z_x}$.
% More generally, we can repeat this process $L$ times, with $L$ sets of hash functions, leading to  $z_x^i = (h_1^i(x),\ldots,h_s^i(x))$ for $i = 1,2,\ldots, L$. Then we learn linear functions $g^i_{z^i_x}$ and approximate $f(x)$ with $g(x) = \sum_{i=1}^L \alpha_i \hat g^i_{z^i_x}(x)$ for scalars $\alpha_1,\ldots, \alpha_L \in \mathbb{R}$. Let $\LSH(d, s, L)$ denote this class of functions. 

%\subsection{Top-K Activations based Routing}



==> Hybrid Sparsity (arxiv)/theory.tex <==
\section{Data-Dependent Sparse Models are more Efficient than Dense Models}
\label{sec:sparse-random-functions}

For a general class of Lipschitz functions, LSH-based learners yield similar $\ell_{\infty}$ error as dense neural networks while making inference significantly more efficient.
It is a common belief in the machine learning community that although many of the datasets we encounter can appear to live in high-dimensional spaces, there is a low-dimensional manifold that contains the inputs. To model this, we assume in our theory that the inputs lie in a $k$-dimensional subspace (a linear manifold) of $\mathbb{R}^d$. Here $k \ll d$.
% \nishanth{TODO: talk about subspace theorem and manifold theorem separately to highlight difference between them}
Theorem ~\ref{thm:main-lipschitz-lsh-ub} shows that the LSH model we propose can learn high-dimensional Lipschitz functions with a low $\ell_{\infty}$ error efficiently when the input comes from a uniform distribution on an unknown low-dimensional subspace. Theorem~\ref{thm:main-lipschitz-ub-manifolds} extends this result to when the input comes from an unknown manifold with a bounded curvature. We present Theorem~\ref{thm:main-lipschitz-lsh-ub} here and defer Theorem~\ref{thm:main-lipschitz-ub-manifolds} to Section~\ref{sec:manifolds-apdx}. All proofs are in the appendix.
% We note here that our proof of Theorem~\ref{thm:main-lipschitz-ub-manifolds} can also be extended to the setting where the input comes from a union of a small number of manifolds, each of bounded curvature. We define manifolds and curvature in Section~\ref{sec:manifolds-apdx}.

\begin{theorem} \label{thm:main-lipschitz-lsh-ub}
For any $f: [-1, 1]^d \to \mathbb{R}$ that is $L$-Lipschitz, and for an input distribution $\mathcal{D}$ that is uniform on a $k$-dimensional subspace in $[-1,1]^d$, an LSH-based learner can learn $f$ to $\epsilon$-uniform error with $O(kL\sqrt{d}^k\log(L\sqrt{d}/\epsilon)/\epsilon^k)$ samples using a hash table of size $O(L\sqrt{d}^k/\epsilon^k)$ with probability $\ge 0.8$.
The total time required for a forward pass on a new test sample is $O(dk\log(L\sqrt{d}/\epsilon))$.
\end{theorem}

The key idea behind this theorem is to use LSH to produce a good routing function. The locality of the points hashed to an LSH bucket gives us a way to control the approximation error. By using a large number of buckets, we can ensure their volume is small. Then, outputting a representative value suffices to locally approximate the target Lipschitz function (since its value changes slowly). The next lemma bounds the size of the sub-regions corresponding to each bucket, as well as bounding the number of non-empty buckets.

%  what do we output if we don't see any training samples? Nearest neighbor within distance eps so we can take an empty bucket and output the value of the nearest neighbor in the training set -- expect to happen rarely as well (not an issue if the num experts much much smaller than num dataset)


% \begin{remark}[Input Distribution Can be Non-Uniform]
% In Theorem~\ref{thm:main-lipschitz-lsh-ub} we assume a uniform distribution on the $k$-dimensional subspace for simplicity. We can generalize the statement to non-uniform distributions as well. Moreover, as long as the minimum probability mass in a bucket is a constant factor away from the maximum probability mass in a bucket the same bounds on the size of the LSH and the number of samples required to learn the function hold asymptotically.
% \end{remark}

%\nishanth{Perhaps the below remark is too bold?}
% \begin{remark}[Input Manifold can be Non-Linear Too]
% Although Theorem~\ref{thm:main-lipschitz-lsh-ub} is stated when inputs lie in a $k$-dimensional subspace of $\mathbb{R}^d$, we can relax this assumption to when inputs lie in a $k$-dimensional non-linear manifold as long as we bound its curvature appropriately.
% \end{remark}

\begin{lemma}\label{lem:lsh-buckets-size}
Consider a Euclidean $\LSH$ model in $d$ dimensions with $Ck$ hyperplanes and width parameter $\epsilon$ where $C$ is a large enough constant. Consider a region $\Gamma$ defined by the intersection of a $k$-dimensional subspace with $[-1,1]^d$. We have that the $\LSH$ model defines a partitioning of $\Gamma$ into buckets. Let  $c$ be a constant. Then, with probability $\ge 0.9$, 
%\cnote{I agree with the reviewer that saying with probability $\ge 1 - \delta$ and having the explicit $\delta$ dependency would be nicer, even though I assume it's probably only a $\log(1/\delta)$ factor}
\begin{enumerate}
    \item Projecting any bucket of the LSH onto $\Gamma$ corresponds to a sub-region with diameter $\le \epsilon/c$.
    \item At most $\left(\frac{2\sqrt{d}}{\epsilon}\right)^{O(k)}$ buckets have a non-empty intersection with $\Gamma$.
\end{enumerate}
\end{lemma}

The above construction assumes knowledge of the dimensionality of the input subspace $k$. Fortunately, any upper bound on $k$ would also suffice. 
%{\color{red} Can we add another sentence about estimating or guessing $k$ since the reviewer asked?} \cnote{There are some empirical values of the effective dimension for MNIST and ImageNet given in Bubeck's Universal Law of Robustness paper (page 3, paragraphs 3 and 4)} 
The table size of the LSH model scales exponentially in $k$ but not $d$. Thus, an LSH-based learner adapts to the dimensionality of the input subspace.


Theorem~\ref{thm:main-lipschitz-lsh-ub} shows that sparsely activated models (using LSH of a certain table size) are powerful enough to approximate and learn Lipschitz functions. Next, we show a complementary nearly matching lower bound on the width required by dense model to approximate the same class of functions. We use an information theoretic argument.
\begin{theorem} \label{thm:dense-lb}
Consider the problem of learning $L$-Lipschitz functions on $[-1,1]^d$ to $\ell_{\infty}$ error $\epsilon$ when the inputs to the function are sampled from a uniform distribution over an unknown $k$-dimensional subspace of $\mathbb{R}^d \cap [-1,1]^d$.
A dense model of width $t$ with a random bottom layer requires 
$$t = \Omega\left(\frac{(\sqrt{d}L)^k}{(C\epsilon)^k}\right),$$
for a constant $C > 0$ to learn the above class of functions. The number of samples required is
$$\Omega\left(\frac{k(\sqrt{d}L)^k\log(2\sqrt{d}L/C\epsilon)}{(C\epsilon)^k}\right).$$
\end{theorem}

Our approach for this theorem is to use a counting argument. We first bound the number of distinct functions, which is exponential in the number of parameters (measured in bits). We then construct a large family of target functions that are pairwise far apart from each other. Hence, if we learn the wrong function, we incur a large error. Our function class must be large enough to represent any possible target function, and this gives a lower bound on the size of the approximating network.

Theorem~\ref{thm:dense-lb} shows a large gap in the time complexity of inference using a dense model and an LSH model. The inference times taken by a dense model vs.~a sparse model differ exponentially in $1/\epsilon$.
\begin{align}
    \textbf{Sparse: } O\left(dk\log(1/\epsilon) \right)  \qquad \text{vs.} \qquad \textbf{Dense: } \Omega\left(d\left(\frac{2\sqrt{d}}{C\epsilon} \right)^k \right)
\end{align}

Overall, the above theorems show that LSH-based sparsely activated networks can approximate Lipschitz functions on a $k$-dimensional subspace. The size and sample complexity match between sparse and dense models, but the sparse models are exponentially more efficient for inference.

% \nishanth{Can we show that gradient descent in the hybrid sparse model actually learns a good representation? This first leads to the question of how exactly is hybrid sparsity enforced while training and inference? IF we can show this separation even with a trainable bottom layer that would be stronger.}
%\textcolor{red}{Another representation Lemma: If the lower layer is trainable, it can project down}



% Conjecture 3: If a function is analytical, with bounded first $t$ derivatives, then by maintaining $(t + k) \choose t$ coefficients per bucket using LSH, one gets a regression function whose error in $\ell_\infty$ is $\le 1/2^k$.


% - Taylor representable with bounded derivatives?
% - What about Fourier representable functions? 
% - What about random functions? 
% - What about Mixture of Gaussians? Is this the same as a random function via Gaussian random field?

% \begin{theorem} Given Gaussian smoothing of a random noise image $f$ (this is a Gaussian random field?), if smoothing kernel size = $\Gamma$, to learn this using a dense layer, we need width = $\Omega(1/R^2)$ (2D image), vs with 1-level LSH we need a table of size $\Omega(1/R^2)$ but only use $1/\epsilon^2$ lookups. Moreover, this is learnable using gradient descent as well. To represent a hash table of size $\Omega(1/R^2)$, we need $\log(1/R)$ hash functions.
% \end{theorem}

% Extension to above Theorem: If the smoothing kernel size $R(x,y)$ is a function of the space as well, then the optimal table size would be $\int_{(x,y)} 1/R(x,y)^2d(x,y)$.



% Observation:

% 1. For parity function on $k$ bits, having less than exponential in $d$ width will not give a time advantage of hybrid sparse layer over a dense layer. Roughly the argument here is that an LSH table of size $2^k$ won’t suffice to compute the parity on $k$ bits if we don’t know the set $A$. what about the range between $2^k$ and $2^d$?
% 2. Parity is reasonably representative of more degree $k$ polynomials (linear combination of parities) and hence focusing on parities could be general enough.
% 3. $\sin(wx) \approx \sgn((w . x) \mod 2)$ in terms of learning difficulty.

% \subsection{Rina's email}
% Let $\rho(x-y)$ be the probability that the points $x,y$ hash to the same bucket which is a function of the distance $|x-y|_2$.

% Consider an infinite width network of several random LSH copies
% Lemma: A function $f(x)$ can be realized if $f(x) = \rho(x) * g(x) = \int g(y) \rho(x-y) dy$
% Proof:
% Consider a two layer LSH based network $f(x)$ where in the upper layer for an LSH cell region $\Gamma$, the weight $g(R) = \int_R g(x) dx$
% Then $E[f(x)] =  \int g(y) \rho(x-y) dy$

% Observation: If we use $1/\epsilon^2$ copies of LSH, then the deviation $f(x)$ will with high probability be $\epsilon |g|_\infty$.

% Now by using Fourier analysis we can find the right $g$ as $G(\omega) = F(\omega)/P(\omega)$

==> dsm_vs_dense.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Data-Dependent Sparse Models are Less Expressive than Dense Models}
\label{sec:lshpower}
First we establish formally that the dense model is strictly more powerful than the sparse model when given the same width. Simple intuition tells this and this is formalized in the form of Lemmas \ref{lem:dense-expresses-lsh} and \ref{lem:lsh-doesnot-express-dense}.
% To start off with, some observations comparing the representation power of LSH tables vs 1-hidden layer ReLU networks (TLDR: When comparing LSH with table size $M$ and dense ReLU network with hidden width $M$, dense ReLU networks are strictly more expressive than LSH tables)
\begin{lemma}
\label{lem:dense-expresses-lsh}
Given a function $f$ which is expressible using a hyperplane-LSH with table size $M$, there exists a two layer ReLU network of hidden width $M$ which computes $f$. For an LSH parameter $\epsilon$, the norm of the weights in the top layer of the ReLU network will grow as $g(1/\epsilon)$.
\end{lemma}
\begin{proof}
Every entry in the table of the LSH model corresponds to a region in $\mathbb{R}^d$ which corresponds to $\log M$ hyper-plane inequalities being satisfied. 
\end{proof}

\begin{lemma}
\label{lem:lsh-doesnot-express-dense}
The other way around does not hold. Can we use a counting argument (info theoretic LB)? Naive argument on total number of parameters used to represent the function won't work as sparse model has equal (or more) total number of parameters.
Easier goal to prove: there exists a function which can be computed exactly in dense model but can't be exactly computed in sparse model.
Nicer goal: exists a function which can be computed exactly in dense model but can't even be approximated well in sparse model.
%The ability to train the bottom layer of the ReLU network will imply a separation between functions computable using LSH vs those computable using ReLU networks. (see Learning Parities with Neural Networks paper)
\end{lemma}
\begin{proof}

\end{proof}

If allowed sparsity level is much smaller than the input dimension $d$, then the sparse layer might have significantly more limited expressive power as compared to the more dense layer.
Consider a simple linear function which depends on only one of the $d$ input coordinates. (e.g. $f(x) = x_0$.)
\begin{enumerate}
\item Case 1: With a random ReLU layer of width $d/\epsilon^2$ followed by a dense layer on top, we get that we can learn this function. In case we remove the ReLU completely this is easier to see. we compute as our final layer weights $\{ 1/w_{0j}\}_{j=1}^{d/\epsilon^2}$. This will ensure that the $x_0$ component is present in all neurons and in the averaging process the coefficients of other coordinates vanish to 0.
What happens with the ReLU present? for each $x$, approximately half of the neurons will be active and the convergence still goes through at the same asymptotic rate. \nishanth{with ReLU present it is not clear that the other coordinates effect will vanish to 0. since they will only show up at second layer if activation is positive. need to think more carefully}
\item Case 2: With random ReLU layer of width $W$ followed by a $k$-sparse final layer, this is much harder. how large does $W$ need to be? \nishanth{unfinished argument}
$k=d$ trivially solves the problem as it reduces to above case.
\item Case 3: With trainable ReLU layer of width W followed by a $k$-sparse final layer, ... TBF
\end{enumerate}





==> neurips_checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}



\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{See sections~\ref{sec:theory-apdx} and~\ref{sec:experiments} }
  \item Did you describe the limitations of your work?
    \answerYes{See Sec.~\ref{sec:sparse-random-functions} and \ref{sec:conclusion}.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{Our work is primarily theoretical, without targeted applications.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{See Section~\ref{sec:sparse-random-functions} and Sections~\ref{sec:manifolds-apdx} and \ref{sec:theory-apdx} of the Appendix.}
        \item Did you include complete proofs of all theoretical results?
    \answerYes{See Section~\ref{sec:sparse-random-functions} and Sections~\ref{sec:manifolds-apdx} and \ref{sec:theory-apdx} of the Appendix.}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
\answerYes{We include details to reproduce all datasets and experiments.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
        \answerYes{Details about our experiments are in Section~\ref{sec:experiments} and Section \ref{sec:experimental-details-apdx} of the Appendix.}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNo{}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerNo{}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{See Section~\ref{sec:experiments}}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
  \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> parities.tex <==
\section{Properties of Learning Parities Problem}
Learning parity on $k$ bits of a $d$-dimensional input has a polynomial sample complexity. Parity without noise is easy both sample complexity wise and computationally. 
Parity with noise is hard to learn efficiently. But it can be learnt with a with linearly many samples and an exponential time algorithm as long as $k < d/\log d (d^k < 2^d)$. (i.e. it is PAC learnable but not PAC learnable efficiently)
BKW is an algorithm for LPN which uses super-polynomial number of samples to learn parities in sub-exponential time.

An observation on the Learning Parities paper \cite{daniely2020learning}:
Their upper bound for 2-layer trainable NN is stylized to work for parity function which is a single monomial once we find the right subset $A$. If we choose a linear combination of parities over all possible $A$ of size $k$ then their upper bound won’t hold.

Questions:
1. Focusing on the parities example, and allowing ourself exponential width in $k$, what is the right time complexity for learning for both dense linear layer vs sparse linear layer?
2. Focusing on parities example again, and allowing a trainable bottom layer what is the time-space tradeoff curve for both dense top layer vs sparse top layer?
